GeomGCL: Geometric Graph Contrastive Learning for Molecular Property Prediction

Recently many efforts have been devoted to applying graph neural networks (GNNs) to molecular property prediction which is a fundamental task for computational drug and material discovery. One of major obstacles to hinder the successful prediction of molecule property by GNNs is the scarcity of labeled data. Though graph contrastive learning (GCL) methods have achieved extraordinary performance with insufficient labeled data, most focused on designing data augmentation schemes for general graphs. However, the fundamental property of a molecule could be altered with the augmentation method (like random perturbation) on molecular graphs. Whereas, the critical geometric information of molecules remains rarely explored under the current GNN and GCL architectures. To this end, we propose a novel graph contrastive learning method utilizing the geometry of the molecule across 2D and 3D views, which is named GeomGCL. Specifically, we first devise a dual-view geometric message passing network (GeomMPNN) to adaptively leverage the rich information of both 2D and 3D graphs of a molecule. The incorporation of geometric properties at different levels can greatly facilitate the molecular representation learning. Then a novel geometric graph contrastive scheme is designed to make both geometric views collaboratively supervise each other to improve the generalization ability of GeomMPNN. We evaluate GeomGCL on various downstream property prediction tasks via a finetune process. Experimental results on seven real-life molecular datasets demonstrate the effectiveness of our proposed GeomGCL against state-of-the-art baselines.

==> section/intro_v0.tex <==
\section{Introduction} \label{sec-introduction}
% 1. property prediction
% 2. molecular representation GNN
% Now - most focused on learning from chemical semantics
% A few focused on learning from geometry, however for small molecules and quantum property prediction
% General graph contrastive learning: advantage and disadvantage: A few focused on molecular contrastive learning to solve the problem. However

% Our proposed model

%\li{The prediction of molecular property has been widely considered as one of the most significant tasks in many relevant fields, such as developing computational chemistry \cite{goh2017deep} and accelerating the process of drug discovery \cite{wu2018moleculenet,chen2018rise}. Accurately predicting the property can help to find out the appropriate chemical molecules with desired characteristics for downstream applications quickly and effectively.}


\zhou{
The prediction of molecular property has been widely considered as one of the most significant tasks in computational drug and material discovery \cite{goh2017deep,wu2018moleculenet,chen2018rise}.
%
Accurately predicting the property can help to evaluate and select the appropriate chemical molecules with desired characteristics for many downstream applications. 
%
Machine learning methods, especially the deep learning methods, have shown great potentials to tackle the molecular property prediction problem  \cite{xiong2019pushing,yang2019analyzing,danel2020spatial,song2020communicative,shui2020heterogeneous,ijcai2021-309}.
}

\li{Recently, with the development of graph neural networks (GNNs) \cite{wu2020comprehensive}, exploring molecular graph learning models for property prediction have become an emerging research area \cite{wieder2020compact}. The fundamental idea is to translate each molecule to a representation vector with powerful GNN encoders, followed by the prediction module for the specific property. Most commonly, since molecules can be represented as graphs, a majority of works aim to learn from topological structures\hide{\cite{xiong2019pushing}}. In this sense, nodes and edges are referred to as atoms and bonds in the molecule, respectively. Most studies focus on applying graph convolution \cite{duvenaud2015convolutional} and graph attention \cite{xiong2019pushing} approaches  to the original chemical graph, which learns from molecular attributes. }

\zhou{With the remarkable success of graph neural networks (GNNs) in various graph-related tasks \cite{wu2020comprehensive}, exploring GNNs for molecular representation learning have been considered as a promising methods for property prediction \cite{wieder2020compact}. The fundamental idea is to  regard the topology of atoms and bonds as a graph, and translate each molecule to a representation vector with powerful GNN encoders, followed by the prediction module for the specific property. A number of efforts have been made from different directions to leverage the special proprieties of molecules by GNNs like   \cite{yang2019analyzing,danel2020spatial,maziarka2020molecule,song2020communicative,ijcai2021-309}.
}



%\hide{The earlier studies focus on applying graph convolution approaches to the original chemical graph \cite{duvenaud2015convolutional}, which learns from molecular attributes. Then standard message passing neural networks \cite{gilmer2017neural} and attentive graph models \cite{xiong2019pushing} are proposed to propagate atomic features on the molecular graph. }

\li{However, different from the general graph, molecules are more complicated with abundant attributes, including bond features and geometric factors. The above methods always ignore such valuable information which can contribute to the property \cite{danel2020spatial,maziarka2020molecule}. Thus, a number of efforts have been made from different directions. On the one side, to leverage the bond attributes, several edge-based message passing models \cite{yang2019analyzing,song2020communicative,ijcai2021-309} employ the node-edge (i.e, atom-bond) interactive scheme to learn the node and edge embeddings together. While such methods can utilize the edge information explicitly, the geometry of the molecule is absent in the process of graph representation learning. }


\zhou{
Along the other line of GNN development, graph contrastive learning (GCL) methods \cite{wu2021self} have shown promising performance in many applications when there is the lack of sufficient labelled data. 
The scarcity of labeled data is just one of major obstacles to hinder the prediction performance of GNN models (and other deep learning models) for molecular property prediction. For example, it usually requires high cost to collect the labelled data for certain computational drug discovery task, which is also a common problem for many tasks in other domains. 
}


\zhou{However, upon the successful application of GCL metohd, there still need a special resarch attention to apply the GCL to molecular properity prediction. Exiting GCL methods adopt design different data augmentation schemes for the graph data without considering the special property of molecule. However, such data augmentation schema   }

On the other side, a handful of researches start to pay more attention to exploiting geometry-based 
deep learning models \cite{atz2021geometric} on molecular graphs, which generally reveal the advantage of combining geometric information. As shown in Figure \ref{fig-dist-angle}, the molecules can be represented as two-dimensional (2D) and three-dimensional (3D) structural graphs. The 2D view derives from the structural formula of a chemical compound, while 3D view is obtained via the conformation generation at the 3D space. The emerging geometric GNN approaches include encoding local inter-atomic distances \cite{maziarka2020molecule}, infusing 3D geometric distances and angles \cite{klicpera_dimenet_2020,shui2020heterogeneous}, or using the original 3D coordinates of atoms \cite{danel2020spatial}. Although the existing geometry-based models can make use of multiple factors from the 2D chemical graph or 3D spatial graph\hide{based on atomic positions}, such single-view framework limits their powerful ability of learning comprehensive representations. 

\liadd{
Nevertheless, effectively exploiting structures of both views for molecular representation in a cooperative manner is a non-trivial problem due to the difference between 2D and 3D geometry in granularity\hide{sparsity} and stability. Fortunately, the complementarity of 2D and 3D views provides great potential to apply the contrastive learning scheme on molecular graphs. Despite the progress made by the recent studies on graph contrastive learning \cite{sun2019infograph,wu2021self}, the designed data augmentation methods could inevitably alter the natural structure of a molecule. Few attempts have been made to consider the molecular domain knowledge \cite{sun2021mocl} to alleviate the problem of random corruption on molecular graphs, which heavily depends on the selected chemical rules.\hide{for better representation learning, which plays a significant role to improve \hide{the }performance.} Therefore, considering that molecular graphs in 2D and 3D views can provide chemical and geometric information at different levels and further complement each other, there is a clear demand to develop a new paradigm for the molecule-driven contrastive learning without changing graph semantics.
\hide{which enables a new paradigm for }
}

To tackle the aforementioned challenges, we propose a novel geometric-enhanced graph contrastive learning model (\model) for molecular property prediction, which is equipped with the adaptive geometric message passing network (\gnn) as well as a contrastive learning strategy to augment the 2D-3D geometric structure learning process. Firstly, we devise the dual-channel geometric learning procedure to adapt the graph aggregation to both views with leveraging distance and angle information at different granularity levels. Secondly, we further aim to make both views \hide{enhance}complement each other for better geometric comprehension\hide{understanding}. Here, we take the molecular geometry into consideration and propose the 2D-3D geometric contrastive scheme to bridge the knowledge gap between geometric structure modeling and graph representation learning without labels. The representative\hide{beneficial} 3D spatial information can be distilled with the guidance of the stable 2D information, which provides the chemical semantics. The fusion of 2D and 3D graphs promotes the proposed \model extract more expressive representation for property prediction. To summarize, the main contributions of our work are as follows:

\begin{itemize}
    \item To the best of our knowledge, we are among the first to develop the contrastive learning method for molecular graphs  based on geometric views. By means of naturally contrasting the 2D and 3D view graphs of one molecule without any random augmentation process, our proposed \model makes the most of the consistent and realistic structures for better representation learning.
    \item The \model employs the dual-channel message passing neural network, which adaptively captures both 2D and 3D geometric information of molecular graphs. The additional spatial regularizer further preserves the relative relation of geometry and improves the performance.
    \item The experiments on seven molecular datasets demonstrate that the proposed model outperforms the state-of-the-art GNN and graph contrastive learning methods.
\end{itemize}


% by means of contrasting 2D and 3D geometric views, 
% under such framework. 

% distill preserve
% highlight, emerging, promising, augmenting beneficial
% are devised to deal with 
% can not deal with/tackle

% In brief, most of the existing literature miss to incorporate the crucial geometric information. To address, Here, we bridge this knowledge gap by, While few attempts have been made to consider xxx, none of these hybrid methods incorporate xxx simultaneously. All the aforementioned methods inspire us to thoroughly explore xxx for pairwise predictions.

%  most of the existing literature miss to incorporate
% Recently, a handful of studies start to pay more attention on exploiting
% In contrast to the research focused on xxx, this work seeks a more nuanced understanding of xxx

% While few attempts have been made to consider xxx, none of these hybrid methods incorporate xxx simultaneously.

